Runaway electron beam formation, vertical motion, termination and wall loads in EU-DEMO

Runaway electron loads onto material structures are a major concern for future large tokamaks due to the efficient avalanching at high plasma currents. Here, we perform predictive studies using the JOREK code for a plausible plasma configuration in the European DEMO fusion power plant with focus on a pessimistic scenario in which a multi mega-ampere runaway electron beam is formed. The work first comprises axisymmetric predictions of runaway electron beam formation in a mitigated scenario and of the simultaneous vertical motion of the beam due to loss of position control. The subsequent runaway electron beam termination triggered by a burst of MHD activity during the course of the vertical motion is then simulated in 3D with the runaway electron fluid self-consistently coupled to the MHD modes. Finally, the resulting deposition pattern of the runaway electrons onto wall structures is calculated with a relativistic test particle approach. This way, the suitability of a possible sacrificial limiter concept for the protection of first wall components is assessed.

==> Model600.tex <==
\section{Model600}

model600 description without vpar 

equations with RE model coupling


\begin{multline}
    \text{RHS}(\psi) = \Biggl\{\frac{\eta}{R}\left(j-\frac{c\,F_{0}}{B\,R}\,n_{RE}-j_{0}-j_{B}\right) + \left[\psi,u\right]-\frac{F_0}{R}\,\partial_{\varphi}u-\eta_{num}(\partial^2_R+\partial^2_Z)j\,+\,
    \\
    \frac{2\tau_{IC}}{\rho_{corr}B^2}\left(\frac{F_0}{R}\right)^2\left(\frac{F_0}{R}\,\partial_\varphi P_e-\left[\psi,P_e\right]\right)\Biggr\} v\,x_{jac}\,\Delta t + \xi\frac{\delta g}{R}\,v\,x_{jac}
\end{multline}
\begin{multline}
    \text{RHS}(u)=\Biggl\{\left[\frac{R^2}{2}|\nabla_{\perp}u|^2,\rho R^2\right]+\left[\rho R^4\omega,u\right]+\left[\psi,j\right]-\frac{F_0}{R}\partial_{\varphi}j-\left[R^2,p\right]+\mu\,R\Delta_{pol}\omega+\partial_R(\mu\,R)\,\partial_R\omega+R\,\partial_Z\mu\,\partial_Z\omega+
    \\
    -2\tau_{IC}R^4\left(\left[P_i,\omega\right]+(\partial_R\partial_Z u)(\partial^2_R-\partial^2_Z)P_i-(\partial_R\partial_Z P_i)(\partial^2_R-\partial^2_Z)u\right)+\partial_R\left(2\tau_{IC}R^3\partial_Z P_i\partial_R u\right)+\partial_Z\left(2\tau_{IC}R^3\partial_Z P_i\partial_Z u\right)
    \\
    +(\partial_R^2+\partial_Z^2)(\mu\,R\,W_{dia})-\partial_R(\mu\,W_{dia}) - \partial_R\left(\frac{d\mu}{dT}R\,W_{dia}\partial_R T_i\right)- \partial_Z\left(\frac{d\mu}{dT}R\,W_{dia}\partial_Z T_i\right)
    \Biggr\}v\,x_{jac}\,\Delta t
    \\
    + \left(\partial_R\left(\frac{1}{R}\right)-\partial^2_R-\partial^2_Z\right)\left[\mu_{num}\left(\partial_R^2\omega+\frac{\partial_R\omega}{R}+\partial^2_Z\omega\right)\right]v\,x_{jac}\,\Delta t
    \\
    +\frac{tgnum_u}{4}\Biggl\{R^3\left[\rho R^2 \left[\omega,u\right]+f_{cons.,u}\,\omega\left[\rho R^2,u\right],u\right]+3 R^2\partial_Z u\left(\rho R^2\left[\omega,u\right]+f_{cons.,u}\,\omega\left[\rho R^2,u\right]\right)\Biggr\}v\,x_{jac}\,(\Delta t)^2
    \\
    +\xi \left[\partial_R(\rho R^3\partial_R\delta u)+\partial_Z(\rho R^3\partial_Z\delta u)\right]v\,x_{jac}-(1-f_{cons.,u})\left[\partial_R(S_0 R^3\partial_R u)+\partial_Z(S_0 R^3\partial_Z u)\right]v\,x_{jac}\,\Delta t
    \\
    + f_{cons.,u}\Biggl\{\xi\left[\partial_R\left(R^3\delta g\partial_R u\right)+\partial_Z\left(R^3\delta g\partial_Z u\right)\right]+\Delta t
    \,\left[\partial_R(A\partial_R u) +  \partial_Z(A\partial_Z u)\right]\Biggr\}v\,x_{jac}
\end{multline}
\begin{equation}
    A = \left(R^2\left[\rho R^2,u\right]-R F_0(\rho\partial_\varphi v_{\parallel}+v_{\parallel}\partial_\varphi\rho)-R^2\rho\left[v_{\parallel},\psi\right]-R^2 v_{\parallel}\left[\rho,\psi\right]\right)
\end{equation}
\begin{equation}
    \text{with:   } S_0 = S_\rho + S_{Pellet} + S_{bg} + S_{imp}
\end{equation}
\begin{equation}
    \text{RHS}(j)=\frac{1}{R}\left(\Delta^* \psi-j\right)v\,x_{jac}
\end{equation}
\begin{equation}
    \text{RHS}(\omega)=R\left(\Delta_{pol}u -\omega\right)v\,x_{jac}
\end{equation}
\begin{multline}
    \text{RHS}(\rho)=R\Biggl\{S_0 + R\left[\rho,u\right]+2 \rho\partial_Z u + \frac{1}{R}\left[\frac{D_{\parallel}+D_{\parallel,sc,num}\tau_{sc}-D_\perp}{B^2\,R}\left(\frac{F_0}{R}\partial_\varphi(\rho-\rho_{imp})+[\rho-\rho_{imp},\psi]\right),\psi\right]
    \\
    +\frac{1}{R}\left[\frac{D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp}}{B^2\,R}\left(\frac{F_0}{R}\partial_\varphi(\rho_{imp})+[\rho_{imp},\psi]\right),\psi\right]
    \\
    +\frac{1}{R}\partial_R\left[D_{\perp}R\,\partial_R(\rho-\rho_{imp})+D_{\perp,imp}R\,\partial_R \rho_{imp}\right]+\partial_Z\left[D_{\perp}\,\partial_Z(\rho-\rho_{imp})+D_{\perp,imp}\,\partial_Z \rho_{imp}\right]
    \\
    -\left(\frac{F_0}{R^2}\partial_{\varphi}(\rho v_{\parallel})+\frac{v_{\parallel}}{R}\left[\rho,\psi\right]+\frac{\rho}{R}\left[v_{\parallel},\psi\right]\right)+4\tau_{IC}\partial_Z P_i+(\rho+\alpha_e\rho_{imp})\left[\rho_n S_{ion}-(\rho-\rho_{imp}) S_{rec}\right]\\
    +\frac{F_0}{R}\,\partial_{\varphi}\left[\frac{D_\parallel+D_{\parallel,sc,num}\tau_{sc}-D_\perp}{B^2\,R^2}\left(\left[\rho-\rho_{imp},\psi\right]+\frac{F_0}{R}\partial_\varphi(\rho-\rho_{imp})\right)\right]+\frac{1}{R^2}\partial_\varphi\left(D_{\perp}\partial_\varphi (\rho-\rho_{imp})\right)
    \\
    +\frac{F_0}{R}\,\partial_{\varphi}\left[\frac{D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp}}{B^2\,R^2}\left(\left[\rho_{imp},\psi\right]+\frac{F_0}{R}\partial_\varphi(\rho_{imp})\right)\right] +\frac{1}{R^2}\partial_\varphi\left(D_{\perp,imp}\partial_\varphi \rho_{imp}\right)
    \Biggr\}v\,x_{jac}\,\Delta t
    \\
    +\xi\delta g R\,v\,x_{jac}-\left(\partial^2_R+\partial^2_Z-\partial_R\left(\frac{1}{R}\right)\right)\left[D_{\perp,num}\,R\,(\partial^2_R\rho+\frac{\partial_R\rho}{R}+\partial^2_Z\rho)\right]v\,x_{jac}\,\Delta t+
    \\
    +\frac{tgnum_\rho}{4}\Biggl\{\left[R^3[\rho,u],u\right]+\left[\frac{v_{\parallel}^2}{R}\left([\rho,\psi]+\frac{F_0}{R}\partial_\varphi\rho\right),\psi\right]+\frac{F_0}{R}\partial_{\varphi}\left(\frac{v_{\parallel}^2}{R}\left[[\rho,\psi]+\frac{F_0}{R}\partial_\varphi\rho\right]\right)\Biggl\}v\,x_{jac}\,(\Delta t)^2\\
    =R\Biggl\{S_0 + R\left[\rho,u\right]+2 \rho\partial_Z u + \nabla\cdot\left[\left(D_{\parallel}+D_{\parallel,sc,num}\tau_{sc}\right)\nabla_{\parallel}(\rho-\rho_{imp})+D_\perp\nabla_{\perp}(\rho-\rho_{imp})\right]\\
    + \nabla\cdot\left[\left(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}\right)\nabla_{\parallel}\rho_{imp}+D_{\perp,imp}\nabla_{\perp}\rho_{imp}\right]\\
    -\left(\frac{F_0}{R^2}\partial_{\varphi}(\rho v_{\parallel})+\frac{v_{\parallel}}{R}\left[\rho,\psi\right]+\frac{\rho}{R}\left[v_{\parallel},\psi\right]\right)+4\tau_{IC}\partial_Z P_i+(\rho+\alpha_e\rho_{imp})\left[\rho_n S_{ion}-(\rho-\rho_{imp}) S_{rec}\right]\Biggr\}v\,x_{jac}\,\Delta t
    \\
    +\xi\delta g R\,v\,x_{jac}-\left(\partial^2_R+\partial^2_Z-\partial_R\left(\frac{1}{R}\right)\right)\left[D_{\perp,num}\,R\,(\partial^2_R\rho+\frac{\partial_R\rho}{R}+\partial^2_Z\rho)\right]v\,x_{jac}\,\Delta t+
    \\
    +\frac{tgnum_\rho}{4}\Biggl\{\left[R^3[\rho,u],u\right]+\left[\frac{v_{\parallel}^2}{R}\left([\rho,\psi]+\frac{F_0}{R}\partial_\varphi\rho\right),\psi\right]+\frac{F_0}{R}\partial_{\varphi}\left(\frac{v_{\parallel}^2}{R}\left[[\rho,\psi]+\frac{F_0}{R}\partial_\varphi\rho\right]\right)\Biggl\}v\,x_{jac}\,(\Delta t)^2
\end{multline}
\begin{multline}
    \text{RHS}(T)=R\Biggl\{S_0 + (\rho+\rho_{imp}\,\alpha_{imp,bis})R\,[T,u]+T\,R[\rho,u]+\alpha_{imp}\,T\,R\,[\rho_{imp},u]+(\rho+\rho_{imp}\,\alpha_{imp})T\,2\gamma\partial_Z u\\
    -(\rho+\rho_{imp}\,\alpha_{imp,bis})\frac{F_0}{R^2}v_{\parallel}\,\partial_{\varphi}T-T\frac{F_0}{R^2}v_{\parallel}(\partial_\varphi\rho+\alpha_{imp}\partial_{\varphi}\rho_{imp})-(\rho+\rho_n\alpha_{imp,bis})\frac{v_{\parallel}}{R}[T,\psi]-T\,\frac{v_{\parallel}}{R}[\rho,\psi]\\
    -T\,\frac{v_{\parallel}}{R}\alpha_{imp}[\rho_{imp},\psi]-(\rho+\alpha_{imp}\rho_{imp})\frac{T}{R}\gamma[v_{\parallel},\psi]-(\rho+\alpha_{imp}\rho_{imp})\frac{T}{R}\gamma\frac{F_0}{R}\partial_{\varphi} v_{\parallel}\\
    + \frac{1}{R}\left[\frac{\chi_{\parallel}-\chi_{\perp}}{R\,B^2}\left(\frac{F_0}{R}\partial_\varphi T + [T,\psi]\right),\psi\right]+\frac{1}{R}\partial_R(\chi_\perp\,R\,\partial_R T)+ \partial_Z(\chi_\perp\partial_Z T)+(\gamma-1)\frac{\eta_{Ohm}}{R^2}\left(j-\frac{c\,F_0}{B\,R}n_{RE}\right)^2\\
    +\frac{\gamma-1}{2}\left(R(\partial_R u)^2+R(\partial_Z u)^2+\frac{1}{R}B^2\,v^2_{\parallel}\right)\left(\left(\rho+\alpha_e\rho_{imp}\right)\rho_n\,S_{ion}+S_{bg}+S_{imp}\right)+\\
    +(\gamma-1)\nu_{\parallel}((\partial_R v_{\parallel})^2+(\partial_Z v_{\parallel})^2)-(\gamma-1)\left[\frac{1}{R}\partial_R\left(R\,v_{\parallel}\nu_{\parallel}\partial_R v_{\parallel}\right)+\partial_Z\left(v_{\parallel}\nu_{\parallel}\partial_Z v_{\parallel}\right)\right]-\xi_{ion}(\rho+\alpha_e\rho_{imp})\rho_n S_{ion}\\
    -(\rho_{corr}+\alpha_e\rho_{imp,corr})\left[\rho_{n,corr}L_{rad,Drays}+(\rho_{corr}-\rho_{imp,corr})L_{rad,Dcont}+frad_{bg}+\rho_{imp,corr}L_{rad}\right]+p_{teleport,ju}\\
    +(\gamma-1)R\left(\rho_{imp}\frac{dE_{ion}}{dT}[T,u]+E_{ion}[\rho_{imp},u]+E_{ion,bg}[\rho-\rho_{imp},u]\right)\\
    -(\gamma-1)\left(\rho_{imp}\frac{dE_{ion}}{dT}\frac{F_0}{R^2}v_{\parallel}\partial_\varphi T+E_{ion}\frac{F_0}{R^2}v_{\parallel}\partial_\varphi\rho_{imp}+E_{ion,bg}\frac{F_0}{R^2}v_{\parallel}\partial_\varphi(\rho-\rho_{imp})\right)\\
    -(\gamma-1)\frac{v_{\parallel}}{R}\left(\rho_{imp}\frac{dE_{ion}}{dT}[T,\psi]+E_{ion}[\rho_{imp},\psi]+E_{ion,bg}[\rho-\rho_{imp},\psi]\right)\\
    +(\gamma-1)E_{ion}\,\rho_{imp}\left(2 \partial_{Z}u-\frac{1}{R}[v_{\parallel},\psi]-\frac{F_0}{R^2}\partial_\varphi v_{\parallel}\right)+(\gamma-1)E_{ion,bg}(\rho-\rho_{imp})\left(2 \partial_{Z}u-\frac{1}{R}[v_{\parallel},\psi]-\frac{F_0}{R^2}\partial_\varphi v_{\parallel}\right)\\
    +(\gamma-1)\frac{1}{R}\left[\frac{E_{ion}\left(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp}\right)}{B^2R}\left(\frac{F_0}{R}\partial_\varphi\rho_{imp}+\left[\rho_{imp},\psi\right]\right),\psi\right]+(\gamma-1)\frac{1}{R}\partial_R\left(R\,E_{ion}\,D_{\perp,imp}\partial_R\rho_{imp}\right)\\
    +(\gamma-1)\partial_Z\left(E_{ion}\,D_{\perp,imp}\partial_Z \rho_{imp}\right)\\
    +(\gamma-1)\frac{1}{R}\left[\frac{E_{ion,bg}\left(D_{\parallel}+D_{\parallel,sc,num}\tau_{sc}-D_{\perp}\right)}{B^2R}\left(\frac{F_0}{R}\partial_\varphi(\rho-\rho_{imp})+\left[\rho-\rho_{imp},\psi\right]\right),\psi\right]\\+\frac{1}{R}(\gamma-1)\partial_R\left(R\,E_{ion,bg}\,D_{\perp}\partial_R(\rho-\rho_{imp})\right)
    +(\gamma-1)\partial_Z\left(E_{ion,bg}\,D_{\perp}\partial_Z (\rho-\rho_{imp})\right)\\
    +\frac{F_0}{R}\partial_\varphi\left[\frac{\chi_{\parallel}-\chi_{\perp}}{R^2\,B^2}\left(\frac{F_0}{R}\partial_\varphi T + \left[T,\psi\right]\right)\right]+\frac{1}{R^2}\partial_\varphi\left(\chi_{\perp}\partial_{\varphi}T\right)\\
    +\frac{\gamma-1}{R} \partial_\varphi\left(F_0\frac{E_{ion}}{B^2R^2}(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp})\left(\frac{F_0}{R}\partial_\varphi\rho_{imp}+[\rho_{imp},\psi]\right)+\frac{E_{ion}}{R}D_{\perp,imp}\partial_{\varphi}\rho_{imp}\right)\\
    +\frac{\gamma-1}{R} \partial_\varphi\left(F_0\frac{E_{ion,bg}}{B^2R^2}(D_{\parallel}+D_{\parallel,sc,num}\tau_{sc}-D_{\perp})\left(\frac{F_0}{R}\partial_\varphi(\rho-\rho_{imp})+[\rho-\rho_{imp},\psi]\right)+\frac{E_{ion,bg}}{R}D_{\perp}\partial_{\varphi}(\rho-\rho_{imp})\right)
    \Biggr\} v\,x_{jac}\,\Delta t\\+ tgnum_T\,(...) + \zeta\,(...) + \chi_{\perp,num}(...)
    \end{multline}
    \begin{multline}
    \text{RHS}(T)=R\Biggl\{S_0 + (\rho+\rho_{imp}\,\alpha_{imp,bis})R\,[T,u]+T\,R[\rho,u]+\alpha_{imp}\,T\,R\,[\rho_{imp},u]+(\rho+\rho_{imp}\,\alpha_{imp})T\,2\gamma\partial_Z u\\
    +(\gamma-1)\nabla\cdot\left(E_{ion}\left(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}\right)\nabla_{\parallel}\rho_{imp}+E_{ion} D_{\perp,imp}\nabla_{\perp}\rho_{imp}\right)\\
    +(\gamma-1)\nabla\cdot\left(E_{ion,bg}\left(D_{\parallel}+D_{\parallel,sc,num}\tau_{sc}\right)\nabla_{\parallel}(\rho-\rho_{imp})+E_{ion,bg} D_{\perp}\nabla_{\perp}(\rho-\rho_{imp})\right)\\
    +\nabla\cdot\left(\chi_{\parallel}\nabla_{\parallel}T+\chi_{\perp}\nabla_{\perp}T\right)+(\gamma-1)\frac{\eta_{Ohm}}{R^2}\left(j-\frac{c\,F_0}{B\,R}n_{RE}\right)^2
    +\frac{\gamma-1}{2}\left(R(\partial_R u)^2+R(\partial_Z u)^2\right)\left(\left(\rho+\alpha_e\rho_{imp}\right)\rho_n\,S_{ion}+S_{bg}+S_{imp}\right)\\
    -\xi_{ion}(\rho+\alpha_e\rho_{imp})\rho_n S_{ion}
    \\
    -(\rho_{corr}+\alpha_e\rho_{imp,corr})\left[\rho_{n,corr}L_{rad,Drays}+(\rho_{corr}-\rho_{imp,corr})L_{rad,Dcont}+frad_{bg}+\rho_{imp,corr}L_{rad}\right]+p_{teleport,ju}\\
    +(\gamma-1)R\left(\rho_{imp}\frac{dE_{ion}}{dT}[T,u]+E_{ion}[\rho_{imp},u]+E_{ion,bg}[\rho-\rho_{imp},u]\right)
    +2(\gamma-1) \partial_{Z}u\left[E_{ion}\,\rho_{imp}+E_{ion,bg}(\rho-\rho_{imp})\right]\\
    + \Biggl\{-(\rho+\rho_{imp}\,\alpha_{imp,bis})\frac{F_0}{R^2}v_{\parallel}\,\partial_{\varphi}T-T\frac{F_0}{R^2}v_{\parallel}(\partial_\varphi\rho+\alpha_{imp}\partial_{\varphi}\rho_{imp})-(\rho+\rho_n\alpha_{imp,bis})\frac{v_{\parallel}}{R}[T,\psi]-T\,\frac{v_{\parallel}}{R}[\rho,\psi]
    \\
    -T\,\frac{v_{\parallel}}{R}\alpha_{imp}[\rho_{imp},\psi]-(\rho+\alpha_{imp}\rho_{imp})\frac{T}{R}\gamma[v_{\parallel},\psi]-(\rho+\alpha_{imp}\rho_{imp})\frac{T}{R}\gamma\frac{F_0}{R}\partial_{\varphi} v_{\parallel}+\frac{\gamma-1}{2\,R}B^2\,v^2_{\parallel}\left(\left(\rho+\alpha_e\rho_{imp}\right)\rho_n\,S_{ion}+S_{bg}+S_{imp}\right)\\
    +(\gamma-1)\nu_{\parallel}((\partial_R v_{\parallel})^2+(\partial_Z v_{\parallel})^2) -(\gamma-1)\left[\frac{1}{R}\partial_R\left(R\,v_{\parallel}\nu_{\parallel}\partial_R v_{\parallel}\right)+\partial_Z\left(v_{\parallel}\nu_{\parallel}\partial_Z v_{\parallel}\right)\right]\\-(\gamma-1)\frac{v_{\parallel}}{R}\left(\rho_{imp}\frac{dE_{ion}}{dT}[T,\psi]+E_{ion}[\rho_{imp},\psi]+E_{ion,bg}[\rho-\rho_{imp},\psi]\right)\\-(\gamma-1)\left(\rho_{imp}\frac{dE_{ion}}{dT}\frac{F_0}{R^2}v_{\parallel}\partial_\varphi T+E_{ion}\frac{F_0}{R^2}v_{\parallel}\partial_\varphi\rho_{imp}+E_{ion,bg}\frac{F_0}{R^2}v_{\parallel}\partial_\varphi(\rho-\rho_{imp})\right)\\
    -(\gamma-1)\left[E_{ion}\rho_{imp}+E_{ion,bg}(\rho-\rho_{imp})\right]\left(\frac{1}{R}[v_{\parallel},\psi]+\frac{F_0}{R^2}\partial_\varphi v_{\parallel}\right)
    \Biggr\}
    %+ \frac{1}{R}\left[\frac{\chi_{\parallel}-\chi_{\perp}}{R\,B^2}\left(\frac{F_0}{R}\partial_\varphi T + [T,\psi]\right),\psi\right]+\frac{1}{R}\partial_R(\chi_\perp\,R\,\partial_R T)+ \partial_Z(\chi_\perp\partial_Z T)
    %\\
    %\\
    %+(\gamma-1)\frac{1}{R}\left[\frac{E_{ion}\left(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp}\right)}{B^2R}\left(\frac{F_0}{R}\partial_\varphi\rho_{imp}+\left[\rho_{imp},\psi\right]\right),\psi\right]+(\gamma-1)\frac{1}{R}\partial_R\left(R\,E_{ion}\,D_{\perp,imp}\partial_R\rho_{imp}\right)\\
    %+(\gamma-1)\partial_Z\left(E_{ion}\,D_{\perp,imp}\partial_Z \rho_{imp}\right)\\
    %+(\gamma-1)\frac{1}{R}\left[\frac{E_{ion,bg}\left(D_{\parallel}+D_{\parallel,sc,num}\tau_{sc}-D_{\perp}\right)}{B^2R}\left(\frac{F_0}{R}\partial_\varphi(\rho-\rho_{imp})+\left[\rho-\rho_{imp},\psi\right]\right),\psi\right]\\+\frac{1}{R}(\gamma-1)\partial_R\left(R\,E_{ion,bg}\,D_{\perp}\partial_R(\rho-\rho_{imp})\right)
    %+(\gamma-1)\partial_Z\left(E_{ion,bg}\,D_{\perp}\partial_Z (\rho-\rho_{imp})\right)\\
    %+\frac{F_0}{R}\partial_\varphi\left[\frac{\chi_{\parallel}-\chi_{\perp}}{R^2\,B^2}\left(\frac{F_0}{R}\partial_\varphi T + \left[T,\psi\right]\right)\right]+\frac{1}{R^2}\partial_\varphi\left(\chi_{\perp}\partial_{\varphi}T\right)\\
    %+\frac{\gamma-1}{R} \partial_\varphi\left(F_0\frac{E_{ion}}{B^2R^2}(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp})\left(\frac{F_0}{R}\partial_\varphi\rho_{imp}+[\rho_{imp},\psi]\right)+\frac{E_{ion}}{R}D_{\perp,imp}\partial_{\varphi}\rho_{imp}\right)\\
    %+\frac{\gamma-1}{R} \partial_\varphi\left(F_0\frac{E_{ion,bg}}{B^2R^2}(D_{\parallel}+D_{\parallel,sc,num}\tau_{sc}-D_{\perp})\left(\frac{F_0}{R}\partial_\varphi(\rho-\rho_{imp})+[\rho-\rho_{imp},\psi]\right)+\frac{E_{ion}}{R}D_{\perp}\partial_{\varphi}(\rho-\rho_{imp})\right)
    \Biggr\} v\,x_{jac}\,\Delta t\\+ tgnum_T\,(...) + \zeta\,(...) + \chi_{\perp,num}(...)
\end{multline}
\begin{multline}
    \text{RHS}(\rho_{imp})=R\Biggl\{\frac{1}{R}\left[(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp})\frac{1}{R\,B^2}\left(\frac{F_0}{R}\partial_\varphi\rho_{imp}+[\rho_{imp},\psi]\right),\psi\right]+\frac{1}{R}\partial_R\left(R\,D_{\perp,imp}\partial_R\rho_{imp}\right)\\
    +\partial_Z\left(D_{\perp,imp}\partial_Z\rho_{imp}\right)+R\,[\rho_{imp},u]+2\rho_{imp}\partial_Z u-\frac{F_0}{R^2}v_{\parallel}\partial_\varphi\rho_{imp}-\frac{v_{\parallel}}{R}[\rho_{imp},\psi]-\frac{F_0}{R^2}\rho_{imp}\partial_\varphi v_{\parallel}-\frac{\rho_{imp}}{R}[v_{\parallel},\psi]\\
    +S_{imp} +\frac{F_{0}}{R}\partial_\varphi\left(\frac{D_{\parallel,imp}-D_{\perp,imp}}{B^2\,R^2}\left(\frac{F_0}{R}\partial_\varphi\rho_{imp}+[\rho_{imp},\psi]\right)\right)+\frac{1}{R^2}\partial_\varphi(D_{\perp,imp}\partial_{\varphi}\rho_{imp})\Biggr\}v\,x_{jac}\,\Delta t+tgnum_{\rho,imp}\left(...\right)\\ + \delta g \left(...\right)-D_{n,\perp,num}\left(...\right)\\
    =R\Biggl\{\nabla\cdot\left[(D_{\parallel,imp}+D_{\parallel,imp,sc,num}\tau_{sc}-D_{\perp,imp})\nabla_{\parallel}\rho_{imp}+D_{\perp,imp}\nabla_{\perp}\rho_{imp}\right]+R[\rho_{imp},u]+2\rho_{imp}\partial_{Z}u+S_{imp}\\
    -\frac{F_0}{R^2}v_{\parallel}\partial_\varphi\rho_{imp}-\frac{v_{\parallel}}{R}[\rho_{imp},\psi]-\frac{F_0}{R^2}\rho_{imp}\partial_\varphi v_{\parallel}-\frac{\rho_{imp}}{R}[v_{\parallel},\psi]
    \Biggr\}v\,x_{jac}\,\Delta t+tgnum_{\rho,imp}\left(...\right)+ \delta g \left(...\right)-D_{n,\perp,num}\left(...\right)
\end{multline}
\begin{multline}
    \text{RHS}(n_{RE})= R\Biggl\{(f_{trit}S_{trit}+f_{compt}S_{compt}+f_{ress}S_{avalanche}) + 2\,n_{RE}\partial_Z u + R\left[n_{RE},u\right]\\ 
-\frac{v_{light,adv}}{F_0}\left([n_{RE},\psi]+\frac{n_{RE}}{R}\partial_Z\psi\right)
    -\frac{v_{light,adv}}{R}\partial_{\varphi}n_{RE}+\frac{1}{R}\left[(D_{\parallel,RE}-D_{\perp,RE})\frac{1}{R\,B^2}\left(\frac{F_0}{R}\partial_\varphi n_{RE}+\left[n_{RE},\psi\right]\right),\psi\right]\\
    +\frac{1}{R}\partial_R\left(R\,D_{\perp,RE}\partial_{R}n_{RE}\right)+\partial_Z\left(D_{\perp,RE}\partial_{Z}n_{RE}\right)
    +\frac{F_0}{R}\partial_{\varphi}\left[\frac{D_{\parallel,RE}-D_{\perp,RE}}{R^2\,B^2}\left(\frac{F_0}{R}\partial_\varphi n_{RE}+[n_{RE},\psi]\right)\right]+\frac{1}{R^2}\partial_\varphi(D_{\perp,RE}\partial_{\varphi}n_{RE})\Biggr\}\\
     +R\zeta\delta g \left(...\right)  + D_{\perp,num}(...) + tgnum_{nRE} (...)\\
     =R\Biggl\{(f_{trit}S_{trit}+f_{compt}S_{compt}+f_{ress}S_{avalanche}) + 2\,n_{RE}\partial_Z u + R\left[n_{RE},u\right]\\ 
-\frac{v_{light,adv}}{F_0}\left([n_{RE},\psi]+\frac{n_{RE}}{R}\partial_Z\psi\right)
    -\frac{v_{light,adv}}{R}\partial_{\varphi}n_{RE}+\nabla\cdot\left(D_{\parallel,RE}\nabla_{\parallel}n_{RE}+D_{\perp,RE}\nabla_{\perp}n_{RE}\right)\Biggr\}\\
     +R\zeta\delta g \left(...\right)  + D_{\perp,num}(...) + tgnum_{nRE} (...)
\end{multline}
\textbf{NB:}
\begin{multline}
\nabla\cdot(D_{\parallel}\nabla_{\parallel}f+D_{\perp}\nabla_{\perp}f)=\frac{1}{R}\partial_R\left(R D_{\perp}\partial_R f\right)+\partial_Z(D_\perp\partial_Z f)+\frac{1}{R}\left[\frac{D_\parallel-D_\perp}{B^2 R}\left([f,\psi]+\frac{F_0}{R}\partial_\varphi f\right),\psi\right]
    \\
    + \frac{1}{R^2}\partial_\varphi\left(D_\perp\partial_\varphi f\right)+\frac{F_0}{R}\partial_\varphi\Biggl\{\frac{D_\parallel-D_\perp}{B^2 R^2}\left([f,\psi]+\frac{F_0}{R}\partial_\varphi f\right)\Biggr\}
\end{multline}
\begin{equation}
    v_{light,adv}=re_{adv,fact}\,v_{light}
\end{equation}
In my case:
\begin{equation}
    \mu_{num},\mu\in \text{const.},\quad tgnum_u=1,\quad\tau_{IC}=0,\quad \tau_{sc}=0,\quad Wdia=0,\quad f_{cons,u}=1,\quad \tau_{sc}=0
\end{equation}
\begin{equation}
    with\_neutrals=.false.\,\implies\,S_{rec}=S_{ion}=0
\end{equation}
\begin{equation}
    re_{adv,fact}=0
\end{equation}

==> Results.tex <==
\section{Physics results}\label{sec:physics}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.8\textwidth]{Fig/Impurities_8e22.png}
\caption{}
\label{}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=1.0\textwidth]{Fig/Impurities_scan.png}
\caption{}
\label{}
\end{figure}



\begin{figure}[h!]
  \centering
  \includegraphics[width=0.8\textwidth]{./Fig/ntor15_0D.png}
\caption{}
\label{}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=1.0\textwidth]{./Fig/poloidal_flux.png}
\caption{}
\label{}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.6\textwidth]{./Fig/Poincare_rho_theta.png}
   \includegraphics[width=0.5\textwidth]{Fig/current_q-profile.png}
\caption{}
\label{}
\end{figure}

==> packages.tex <==
\usepackage[utf8]{inputenc}
%\usepackage{amsmath}
\usepackage{mathrsfs,amsmath} 
\usepackage{systeme}
\usepackage{mathtools}
\usepackage{authoraftertitle}
\usepackage{physics}
\usepackage{hyperref}
\usepackage{url}
\usepackage{subcaption} % !!! for subfigures and others !!!
\setlength{\textwidth}{16.2cm}
\setlength{\oddsidemargin}{0.1cm}
\setlength{\evensidemargin}{-0.3cm}
\setlength{\topmargin}{0cm}
\setlength{\textheight}{22cm}\setlength{\marginparwidth}{2cm}

\usepackage{lipsum}
\usepackage[draft]{todonotes} 
\usepackage{chngcntr}
\usepackage{tikz-cd}
\usepackage{chemfig}
%\usepackage{samepage}
\usepackage{needspace}
%\usepackage{biblatex}
%\usepackage[paperwidth=5in,paperheight=7in]{geometry}
\usepackage{cleveref}
\usepackage[absolute]{textpos}
\usepackage{dirtytalk}


\usepackage{mathrsfs,amsmath} 


\usepackage[section]{placeins}
\usepackage{subfiles}


\usepackage[math]{cellspace}

\usepackage{graphicx,epsf}
\usepackage{array,multirow}
\usepackage{bm}
\usepackage{comment}
